Language-guided Task Adaptation for Imitation Learning

We introduce a novel setting, wherein an agent needs to learn a task from a demonstration of a related task with the difference between the tasks communicated in natural language. The proposed setting allows reusing demonstrations from other tasks, by providing low effort language descriptions, and can also be used to provide feedback to correct agent errors, which are both important desiderata for building intelligent agents that assist humans in daily tasks. To enable progress in this proposed setting, we create two benchmarks -- Room Rearrangement and Room Navigation -- that cover a diverse set of task adaptations. Further, we propose a framework that uses a transformer-based model to reason about the entities in the tasks and their relationships, to learn a policy for the target task

==> LaTeX/retail_lang_data.tex <==
\begin{table*}
\caption{Examples of template-generated and natural language descriptions collected using AMT.}
\small
\begin{tabular}{l p{0.435\textwidth}p{0.435\textwidth}}
\hline
% \vspace{2pt}
  & \Tstrut {\textbf{Template}}                                              & {\textbf{Natural language paraphrase}}\Bstrut                    \\
\hline
1.
& \Tstrut go further away from the metallic table
& Increase your distance from the metallic table.
\Bstrut \\ \hline
2.
& \Tstrut go closer to the foldable light
& Move in the direction of the light that is foldable
\Bstrut \\ \hline
3.
& \Tstrut go to the opposite side of the corner light
& Move across from the corner light.
\Bstrut \\ \hline
4.
& \Tstrut move the large chair one unit farther from the wide couch
& Increment the distance of the big chair from the wide couch by one.
\Bstrut \\ \hline
% 5.
% & \Tstrut Move the blue disk to the final position of the red tall cylinder, and vice versa.
% & Swap the ending positions of the red cylinder and blue disc
% \Bstrut \\ \hline
% 6.
% & \Tstrut Skip the first step.
% & Omit the beginning step
% \Bstrut \\ \hline
5.
& \Tstrut move corner table two units further left and metallic shelf one unit further backward
& slide the corner table two units left and move the metal shelf a single unit back
\Bstrut \\ \hline
6.
& \Tstrut move the large table to where the large sofa was moved, and vice versa
& swap the place of the table with the sofa
\Bstrut \\ \hline
% 7.
% & \Tstrut Move blue tall block from top right to bottom left after the second step.
% & Move blue tall square from upper option to base left after the subsequent advance.
% \Bstrut \\ \hline
% 10.
% & \Tstrut Move blue tall cylinder from bottom left to middle left after the first step.
% & For the second step move the blue tall cylinder to the middle left
% \Bstrut \\ \hline
% 7.                            & \Tstrut Don't move green flat block from middle right to bottom left.                      & Do not move green flat block.                                               \Bstrut \\ \hline
% 8.                            & \Tstrut Move blue tall cylinder from bottom left to middle left after the first step.      & For the second step move the blue tall cylinder to the middle left          \Bstrut \\ \hline
% 9.                            & \Tstrut In the end, move blue disk from middle right to bottom right.                      & On the final step put the blue disc into the bottom right position          \Bstrut \\ \hline
% 10.                           & \Tstrut Move the green cylinder to where blue flat block was moved.                        & Put the green cylinder in the spot vacated by the flat blue block           \Bstrut \\ \hline
% 11.                           & \Tstrut In the third step, move the green tall cylinder from top left to bottom right.     & Put the green cylinder in the bottom right corner                           \Bstrut \\ \hline
% 12.                           & \Tstrut Move blue tall block from top right to bottom left after the second step.          & Move blue tall square from upper option to base left after the subsequent advance.  \Bstrut \\ \hline
\end{tabular}
\label{tbl:retail-syn-nat-examples}
\end{table*}
